TranSHER: Translating Knowledge Graph Embedding with Hyper-Ellipsoidal Restriction

Knowledge graph embedding methods are important for the knowledge graph completion (or link prediction) task. One existing efficient method, PairRE, leverages two separate vectors to model complex relations (i.e., 1-to-N, N-to-1, and N-to-N) in knowledge graphs. However, such a method strictly restricts entities on the hyper-ellipsoid surfaces which limits the optimization of entity distribution, leading to suboptimal performance of knowledge graph completion. To address this issue, we propose a novel score function TranSHER, which leverages relation-specific translations between head and tail entities to relax the constraint of hyper-ellipsoid restrictions. By introducing an intuitive and simple relation-specific translation, TranSHER can provide more direct guidance on optimization and capture more semantic characteristics of entities with complex relations. Experimental results show that TranSHER achieves significant performance improvements on link prediction and generalizes well to datasets in different domains and scales. Our codes are public available at https://github.com/yizhilll/TranSHER.

==> res_figures/top_score_comparison.tex <==
\begin{figure}[hbt!]
\centering
\begin{subfigure}{0.4\linewidth}
\centering
\includegraphics[width=0.4\linewidth, height=60pt]{example-image} 
\caption{Original}\label{translation_top_scores:a}
\end{subfigure}
\begin{subfigure}{0.4\linewidth}
\centering
\includegraphics[width=0.4\linewidth, height=60pt]{example-image} 
\caption{Imposter}\label{translation_top_scores:b}
\end{subfigure}

\begin{subfigure}{0.4\linewidth}
\centering
\includegraphics[width=0.4\linewidth, height=60pt]{example-image} 
\caption{Imposter}\label{translation_top_scores:c}
\end{subfigure}
\begin{subfigure}{0.4\linewidth}
\centering
\includegraphics[width=0.4\linewidth, height=60pt]{example-image} 
\caption{Imposter}\label{translation_top_scores:d}
\end{subfigure}


\caption{Top-$N$ Score Statistics in FB15k-237 Validation Results. The triplets in the validation set are selected and grouped if both TransHER and baseline model PairRE acquire rankings higher than top-$N$. Expectation of Top-N Score Standard Deviation (Fig.~\ref{translation_top_scores:c},~\ref{translation_top_scores:d})}
    
\label{translation_top_scores}
\end{figure}

==> res_tables/bias_initialization_ablation.tex <==
\begin{table}[hbt!]


\centering
\scalebox{0.75}{
    \begin{tabular}{c|c|cccc}
    \hline
    % \textbf{Dataset} & Translation & \multicolumn{4}{c}{\textbf{FB15k-237}} \\
    % \textbf{Metric} & Initialization & MRR & HIT@1 & HIT@3 & HIT@10 0 \\
   \multirow{2}{*}{\textbf{Model}} & \multirow{2}{*}{\textbf{Init.}} &  \multicolumn{4}{c}{\textbf{Metric}} \\ \vspace{3pt}
     &  & MRR & HIT@1 & HIT@3 & HIT@10 \\
    \hline \hline \vspace{3pt}
    PairRE & N/A & .351 & .256 & .387 & .544 \\ 
    \hline \vspace{3pt}
    \multirow{4}{*}{TransHER} & $\mathcal{N}$  & .245 & .165 & .265 & .411 \\  \vspace{3pt}
      & $
\mathcal{U}_{\gamma}$ & .347 & .255 & .381 & .533 \\  \vspace{3pt}

     & $\mathcal{U}_{X}$& .353 & .259 & .389 & .544\\  \vspace{3pt}
     & $\mathcal{N}_{X}$ & \textbf{.357} & \textbf{.262} & \textbf{.394} & \textbf{.548} \\
    \hline
    \end{tabular}
}
% \large
\caption{A Study of Different Initialization Strategied for Relation-Specific Translation on FB15k-237.}
\label{bias_initialization}
\end{table}

==> res_tables/rel_type_fb15k_result.tex <==
\begin{table}[htbp]

\caption{Evaluation Result on FB15k. TransE, ComplEX and RotatE are taken from \cite{sun2018rotate}. PairRE* refers to our reproduced version.}


\scalebox{0.75}{
    \begin{tabular}{c|cccc|cccc}
    \hline
    \textbf{Rel. Type} & 1-to-1 & 1-to-N & N-to-1 & N-to-N & 1-to-1 & 1-to-N & N-to-1 & N-to-N \\
    \hline \hline
    % \textbf{Dataset} & \multicolumn{8}{c}{FB15k} \\ \hline
    \textbf{Task} & \multicolumn{4}{c|}{\textbf{Prediction Head (MRR)}} & \multicolumn{4}{c}{\textbf{Prediction Tail (MRR)}}  \\
    \hline 
    TransE & .701 & .912 & .424 & .737 & .701 & .561 & .894 & .761  \\
    ComplEx & .832 & .914 & .543 & .787 & .826 & .661 & .869 & .800 \\
    RotatE & \textbf{.878} & .934 & .465 & .803 & \textbf{.872} & .611 & .909 & .832  \\
    PairRE* & .863 & \textbf{.936} & .547 & .813 & .856 & .674 & \textbf{.917} &  .843 \\
    TransHER & .832 & .929 & \textbf{.588} & \textbf{.851} & .826 & \textbf{.703} & .900 &  \textbf{.856} \\
    \hline
    \textbf{Task} & \multicolumn{4}{c|}{\textbf{Prediction Head (HIT@10)}} & \multicolumn{4}{c}{\textbf{Prediction Tail (HIT@10)}} \\
    \hline 
    TransE & .894 & .972 & .567 & .880 & .879 & .671 & .964 & .910  \\
    ComplEx & .939 & .969 & .692 & .893 & .938 & .823 & .952 & .910  \\
    RotatE & .922 & .967 & .602 & .893 & .923 & .713 & .961 & .922  \\
    PairRE* & .921 & .972 & .686 & .896 & .945 & .806 & .964 & .928  \\
    TransHER & .892 & .967 & .668 & .896 & .893 & .807 & .955 &  .925 \\
    \hline
    \end{tabular}
}

% FB15k version
% \scalebox{1.0}{
%     \begin{tabular}{c|cccc|cccc}
%     \hline
%     Dataset & \multicolumn{4}{c|}{MRR on FB15k (head)} & \multicolumn{4}{c}{MRR on FB15k (tail)}\\
%     Rel. Type & 1-1 & 1-N & N-1 & N-N & 1-1 & 1-N & N-1 & N-N \\
%     \hline \hline
%     baseline &  &  &  &  &  &  &  &  \\
%     baseline &  &  &  &  &  &  &  &  \\
%     baseline &  &  &  &  &  &  &  &  \\
%     PairRE & - &  &  &  & - &  &  &  \\
%     \hline
%     PairRE-B & - &  &  &  & - &  &  &  \\
%     % PairRE-B + N &  &   &   &   &   &   &   &   \\
%     \hline
%     \end{tabular}

% }
\label{tbl_rel_type_fb15k_result}
\end{table}

==> res_tables/rel_type_stats.tex <==
\begin{table}[htbp]
% \small

\caption{Relation Type Statistics of Analyzed Datasets. The number of triplets in training data and the number of different relation types are counted.}

\scalebox{0.85}{
    \begin{tabular}{c|cc|cc|cc|cc}
    \hline 
    \multirow{2}{*}{Rel. Type} & \multicolumn{2}{c|}{1-to-1} & \multicolumn{2}{c|}{1-to-N} &  \multicolumn{2}{c|}{N-to-1} & \multicolumn{2}{c}{N-to-N} \\
        & Trp. & Rel. & Trp. & Rel. & Trp. & Rel. & Trp. & Rel.  \\
    \hline \hline
    FB15k-237 & 4.3k & 17 & 12.5k & 26 &  50.6k & 86 & 204.7k & 108 \\
    DB100K  & 15.5k & 158 & 17.0k & 54 &  131.7k & 163 & 433.4k & 95 \\
    \hline
    \end{tabular}
}


\label{tbl_rel_type_stats}

\end{table}
% Only train

% There are 4278 triples for 17 1-1 relation in ./data/FB15k-237 dataset.
% There are 12536 triples for 26 1-n relation in ./data/FB15k-237 dataset.
% There are 50635 triples for 86 n-1 relation in ./data/FB15k-237 dataset.
% There are 204666 triples for 108 n-n relation in ./data/FB15k-237 dataset.

% There are 15469 triples for 158 1-1 relation in ./data/DB100K dataset.
% There are 17029 triples for 54 1-n relation in ./data/DB100K dataset.
% There are 131660 triples for 163 n-1 relation in ./data/DB100K dataset.
% There are 433414 triples for 95 n-n relation in ./data/DB100K dataset.

==> res_tables/relation_definition.tex <==
\begin{table}[htbp]
% \vspace{-2mm}
\caption{Definition of Knowledge Graph Relation Types.}
\vspace{-2mm}
\begin{tabular}{c|c|c|c|c}
\hline
\textbf{Rel. Type} & \multicolumn{1}{c|}{\textbf{1-to-1}} & \multicolumn{1}{c|}{\textbf{1-to-N}} & \multicolumn{1}{c|}{\textbf{N-to-1}} & \multicolumn{1}{c}{\textbf{N-to-N}} \\
\hline \hline
heads per tail & $< 1.5$ & $< 1.5$ & $\geq 1.5$ & $\geq 1.5$ \\
tails per head & $< 1.5$ & $\geq 1.5$ & $< 1.5$ & $\geq 1.5$ \\
\hline
\end{tabular}
% \vspace{-2mm}
\label{tbl_rel_definition}
\end{table}
